Applying Large Language Models to Issue Classification: Revisiting with Extended Data and New Models

Effective prioritization of issue reports in software engineering helps to optimize resource allocation and information recovery. However, manual issue classification is laborious and lacks scalability. As an alternative, many open source software (OSS) projects employ automated processes for this task, yet this method often relies on large datasets for adequate training. Traditionally, machine learning techniques have been used for issue classification. More recently, large language models (LLMs) have emerged as powerful tools for addressing a range of software engineering challenges, including code and test generation, mapping new requirements to legacy software endpoints, and conducting code reviews. The following research investigates an automated approach to issue classification based on LLMs. By leveraging the capabilities of such models, we aim to develop a robust system for prioritizing issue reports, mitigating the necessity for extensive training data while also maintaining reliability in classification. In our research, we developed an LLM-based approach for accurately labeling issues by selecting two of the most prominent large language models. We then compared their performance across multiple datasets. Our findings show that GPT-4o achieved the best results in classifying issues from the NLBSE 2024 competition. Moreover, GPT-4o outperformed DeepSeek R1, achieving an F1 score 20% higher when both models were trained on the same dataset from the NLBSE 2023 competition, which was ten times larger than the NLBSE 2024 dataset. The fine-tuned GPT-4o model attained an average F1 score of 80.7%, while the fine-tuned DeepSeek R1 model achieved 59.33%. Increasing the dataset size did not improve the F1 score, reducing the dependence on massive datasets for building an efficient solution to issue classification.

==> Tables/IPMA.tex <==
\begin{table}[!ht]
\centering

\caption{IMPA: Performance referred to Belonging to the Team}
\vspace{-3mm}
\label{tab:ipma}

\begin{tabular}{cc
                }

\hline


%& {\makecell{Power\\ Distance \\ (n=182) \\ \textit{R}\textsuperscript{2} 0.519}} & {\makecell{No Power\\ Distance \\ (n=225) \\  \textit{R}\textsuperscript{2} 0.396} } \\ 
%& \multicolumn{2}{c}{Gender} & {Orig.}\\
%\cmidrule(l){2-3}%\cmidrule(l){4-4}
%& {\makecell{Seg.1\\Intrins.\\Motiv.}} & {\makecell{Seg.2\\Extrins.\\Mot.}} & {\makecell{All}}\\
%Group & {Men} & {Women} & {All}\\
%\midrule
%Sample size (N) & {9,867} & {3,877} & {13,477}\\
%\addlinespace

%\addlinespace
%SRMR fit measure %(\textit{R}\textsuperscript{2}) 
%& .06 & .07\\
%\addlinespace
%GoF fit measure %(\textit{R}\textsuperscript{2}) 
%& .74 & .92\\
%\addlinespace
{Latent Construct} & {Performance (\%))} \\
\hline
\hangindent1em Work Appreciation & %\bfseries{77.22\%}  & {75.05\%} & 
{77.13\%}\\
%\midrule
%SB1 & {71.65\%} & {68.97\%} & {70.90\%}\\
%SB2 & {79.98}\% & {78.30}\% & {79.60\%}\\
%SB3 & {78.02}\% & {75.47}\% & {77.30}\%\\
%\midrule
\hangindent1em Psychological Safety & 
%{78.33\%} & \bfseries{75.81\%} & 
{78.56\%}\\ 
%\midrule
%PS1 & {73.41\%} & {70.79\%} & {72.67\%}\\
%PS2 & \bfseries {83.17\%} & \bfseries {82.26\%} & \bfseries {82.92\%}\\
%PS3 & {80.70\%} & {76.50\%} & {79.52\%}\\
%PS4 & {75.30\%} & {72.18\%} & {74.42\%}\\ 
\hangindent1em Belonging to the Team & 
{85.89\%}\\ 
\hline

\end{tabular}

\end{table}


==> Tables/IPMA2.tex <==
\begin{table}[!ht]
\centering

\caption{IPMA: Importance (Effects) referred to Belonging to the Team}
\vspace{-3mm}
\label{tab:ipma2}

\begin{tabular}{lccc}

\hline


& \multicolumn{2}{c}{Role} & \\
\hline
& {Leaders} & {Non-Leaders} & {All}\\

\hline
\hangindent1em Work Appreciation & {.360}  & {.399}  & {.392}\\
\hline
WA1 & {.122} & {.140} &{.137}\\
WA2 & {.172} & \bfseries{.202} & \bfseries{.197}\\
WA3 & \bfseries{.174} & {.176} & {.176}\\
\hline
\hangindent1em Psychological Safety & {.417} & {.407}  & {.410}\\ 
\hline
PS1 & {.144} & {.138} & {.139}\\
PS2 &  {.148} & \bfseries{.156} & {.156}\\
PS3 & {.121} & {.119} & {.120}\\
PS4 & \bfseries{.149} & {.144} & {.145}\\ 

\hline

\end{tabular}

\end{table}

==> Tables/cross_loadings.tex <==
\begin{table*}[!ht]
\footnotesize
\centering
\caption{Cross loadings of indicators on the constructs}
\vspace{-3mm}
\label{tab:cross_loadings}
\begin{tabular}{p{0.2cm}
                p{10cm}
                p{8mm}
                p{8mm}
                p{8mm}}
\hline
& & {Work App.} & {Psyc. Safety} & {Belonging to the Team}\\
\hline
WA1 & I have found a reasonable balance between what I contribute and what I get in return & \textbf{.708} & .410 & .376 \\
WA2 & My leaders recognize my work & \textbf{.816} & .458 & .541 \\
WA3 & My contributions make a difference to the company 
& \textbf{.765} & .458 & .484 \\

\hline
PS1 & I feel safe sharing bad news with my team
& .363 & \textbf{.729} & .461 \\
PS2 & I can be myself at TechCom
& .463 & \textbf{.755} & .515 \\
PS3 & I feel safe reporting improper behaviors such as discrimintaion or harassment 
& .368 & \textbf{.668} & .397 \\
PS4 & I feel safe speaking up and taking risks
& .484 & \textbf{.762} & .479 \\

\hline
BL1 & I can trust people in my team
& .502 & .518 & \textbf{.801}\\
BL2 & I feel accepted by my co-workers
& .470 & .465 & \textbf{.778} \\
BL3 & I feel my co-workers value my opinion &
.553 & .574 & \textbf{.826}\\
BL4 & I have a good relationship with my team &
.467 & .491 & \textbf{.820}\\

\hline

\end{tabular}
\end{table*}

==> Tables/demographics.tex <==
\begin{table}[!t]
\centering
\caption{Demographics of respondents (n=10,781)}
%\vspace{-3mm}
\label{tab:demographics}

\begin{tabular}{p{5cm}
                c
                c}
\hline
Attribute & {N} & {Percentage}\\


\hline
\multicolumn{3}{c}{Country}\\
\hline
Colombia & 2,582 & {23.9\%} \\
India & 2,163 & {20.1\%} \\
Argentina & 1,989 & {18.4\%} \\
Mexico & 1,496 & {13.9\%} \\
Chile & 709 & {6.6\%} \\
Peru & 532 & {4.9\%} \\
Uruguay & 359 & {3.3\%} \\
Brazil & 300 & {2.8\%} \\
Spain & 166 & {1.5\%} \\
USA & 160 & {1.5\%} \\
Romania & 88 & {0.8\%} \\
Ecuador & 82 & {0.8\%} \\
Costa Rica & 72 & {0.7\%} \\
Belarus & 39 & {0.4\%} \\
UK & 25 & {0.2\%} \\
Canada & 8 & {0.1\%} \\
Poland & 6 & {0.1\%} \\
Denmark & 4 & {0.0\%} \\
France & 1 & {0.0\%} \\

\hline
\multicolumn{3}{c}{Role}\\
\hline

Developers & 5,319 & 49.3\% \\
Testers & 1,904 & 17.7\% \\
Project or Product Manager & 1,496 & 13.9\% \\
System Administrator & 652 & 6.0\% \\
Business Analyst & 525 & 4.9\% \\
UX or Design & 457 & 4.2\% \\
Database Administrator & 428 & 4.0\% \\


\hline
\multicolumn{3}{c}{Organizational Tenure}\\
\hline

Less than 1 year & 726 & 6.7\%\\
1-3 years & 7,492 & 69.5\% \\
4-5 years & 1,415 & 13.2\% \\
Over 5 years & 1,148 & 10.6\% \\

\hline
\multicolumn{3}{c}{Gender}\\
\hline

Men & 8,185 & 75.9\% \\
Women & 2,596 & 24.1\% \\

%\hline
%\multicolumn{3}{c}{Age}\\
%\hline

%{18-24} & 782 & xx\% \\
%{25-34} & 6968 & xx\% \\
%{35-44} & 4663 & xx\% \\
%{45+} & 1244 & xx\% \\

%\midrule
%\multicolumn{3}{c}{Tenure at the company}\\
%\midrule
%Less than 6 months & 1677 & 12.6\%\\
%6 months to 1 year & 2812 & 21.1\%\\
%1 year to 3 years & 5586 & 41.9\%\\
%3 years to 5 years & 1594 & 11.9\%\\
%Over 5 years & 1674 & 12.3\& \\

\hline

\end{tabular}

\end{table}

==> Tables/internal_consistency.tex <==
\begin{table}[!hb]
\centering
\caption{Internal Consistency Reliability}
%\vspace{-3mm}
\label{tab:internal_consistency_reliability}
%\robustify{\bfseries}

\begin{tabular}{p{3.5cm}
                c
                c
                c}
\hline
& {Cronbach's Alpha} & {CR} & {AVE}\\
\hline
Work Appreciation & .647 & .808 & .584\\
Psychological Safety & .707 & .820 & .532\\
Belonging to the Team & .821 & .882 & .651\\
\hline


\end{tabular}
\end{table}

==> Tables/mga.tex <==
\begin{table}[!ht]
\centering

\caption{Multi-Group Analysis: coefficients marked with $*$ are statistically significant; gray lines show a significant difference between groups (i.e. leaders/non-leaders)}
\vspace{-10px}
\label{tab:mga}

\begin{tabular}{lccc}

\hline

& \multicolumn{2}{c}{Role} & {Orig.}\\
\hline
%\cmidrule(l){4-4}
%& {\makecell{Seg.1\\Intrins.\\Motiv.}} & {\makecell{Seg.2\\Extrins.\\Mot.}} & {\makecell{All}}\\
Group & {Leaders} & {Non-Leaders} & {All}\\
\hline
Sample size (N) & {1,496} & {9,285} & {10,781}\\
%\addlinespace

%\addlinespace
%SRMR fit measure %(\textit{R}\textsuperscript{2}) 
%& .06 & .07\\
%\addlinespace
%GoF fit measure %(\textit{R}\textsuperscript{2}) 
%& .74 & .92\\
%\addlinespace
\hline
Belonging to the Team (\textit{R}\textsuperscript{2}) & .474 & .516 & .509\\
%\addlinespace


\hline 
H1. Work App. $\rightarrow$ Belonging & .360* & .399*  & .392*\\ 

H2. Psych. Safety  $\rightarrow$ Belonging & .417* & .407*  & .410*\\ 

\hline
Control Variables\\
\hline


\rowcolor{lightgray}\hangindent1em Gender (women) $\rightarrow$ Belonging &   {\textbf{-.015}} & {\textbf{-.121*}} & .010*\\

\hangindent1em Org. Tenure $\rightarrow$ Belonging &  .010 & .018* & .018*\\

\hangindent1em Power Distance $\rightarrow$ Belonging & -.039 & -.071* & -.071*\\

\hline

\end{tabular}
\vspace{-3mm}
\end{table}


==> Tables/path_analysis.tex <==
\begin{table}[!t]
%\footnotesize
\centering
\caption{Standarized path coefficients, standard deviations, confidence intervals, and p-values. * means statistically significant}
\vspace{-3mm}
\label{tab:path_analysis}


\begin{tabular}{lcccc}
\hline
& {\textit{B}} & {SD} & {95\% CI} & p\\
\hline

H1. Work App.$\rightarrow$ Belonging & .392* & .009 & (.37, .41) & .010\\

H2. Psyc. Safety $\rightarrow$ Belonging & .410* & .010 & (.39, .43) & .000\\


\hline
Control Variables\\
\hline
Gender (women)$\rightarrow$ Belonging & -.010* & .002* & (-.13, -.07) & .000\\
Power Distance$\rightarrow$ Belonging & -.071* & .006* & (-.08, -.06) & .000\\
Org. Tenure$\rightarrow$ Belonging & .018* & .006* & (.00, .03) & .000\\



\hline


\end{tabular}
\vspace{-3mm}\end{table}
